Clustering and synchronization analysis of Networks of Bistable Systems

This paper studies the dynamics of a network of diffusively-coupled bistable systems. Under mild conditions and without requiring smoothness of the vector field, we analyze the network dynamics and show that the solutions converge globally to the set of equilibria for generic monotone (but not necessarily strictly monotone) regulatory functions. Sufficient conditions for global state synchronization are provided. Finally, by adopting a piecewise linear approximation of the vector field, we determine the existence, location and stability of the equilibria as function of the coupling gain. The theoretical results are illustrated with numerical simulations.

==> extra.tex <==
\paragraph{Why Piecewise Affine Models}
To understand the dynamics of Gene Regulatory Networks, different type of models with different levels of complexities have been developed in the literature. The most common model of interactions between the different species in the network is described by means of nonlinear sigmoid shaped functions.
In many cases, especially when transcription factors bind with high degree of cooperativity, sigmoid regulatory functions can be approximated using step functions \cite{alon2006introduction}. This approximation leads to a series of qualitative models of the network dynamics, ranging from Boolean Networks to Piecewise Affine models.  The Piecewise Affine dynamics approach, model efficiently several distinct nonlinear dynamical behaviors, such as, multistability or oscillatory behaviors. Compared to the smooth counterpart, the piecewise affine modeling brings a lot of advantages for the analysis. For piecewise affine systems modeling, the dynamics is linear affine in each domain, therefore the dynamics and the computation of equilibria is simplified (as, e.g., in \cite{chaves2019coupling}), but not always comes with the results typical of smooth systems.

Furthermore, we compare this approach with the synchronization analysis based on the theory on cocoercive I/O systems. Such a theory allows some additional flexibility for the conditions on the coupling topologies but it is limited to the study of 'full synchronization', i.e. study of the conditions on the coupling gain to ensure global synchronization of the network, sometimes with results unnecessarily conservative. 

\paragraph{Networked System}
The network motifs described above are often not isolated but interact through a common shared medium (\textit{quorum sensing} \cite{miller2001quorum}, \cite{nikolaev2016quorum}) or through diffusive coupling \cite{silver1996diffusible}, \cite{ali2019multi}.
A natural question that occurs is: what is the role of the coupling in defining the dynamics of the overall network? Are the original steady states preserved and what is the global dynamics of the network when coupling is added? Is the convergence to the original equilibria preserved or destroyed by the addition of coupling?  
For instance, a network of globally asymptotically stable subsystems connected by diffusive coupling may exhibit oscillatory behaviours \cite{pogromsky1999diffusion}.  


\paragraph{Extra equations}


\begin{equation}
	\dot{x} = F(x) = - (\Gamma \otimes I_N + L)x + A \otimes I_n G(x),\ 
	\label{eq:dynamics}
\end{equation}
where 
\begin{equation*}
	G(x) \hspace{-1mm}= \hspace{-1mm} [x_{1,1},\ldots, x_{1,N}, g(x_{2,1}), \ldots, g(x_{2,N}), ]^T
\end{equation*} and
\[
L = \begin{bmatrix}
	L_1 & 0 \\
	0 & 0
\end{bmatrix},\ \Gamma = \begin{bmatrix}
	\gamma_1 & 0 \\
	0 & \gamma_2 
\end{bmatrix},\ A= \begin{bmatrix}
	0 & V_1 \\
	V_2 & 0
\end{bmatrix}.
\]
The matrix $L_1$ is the symmetric Laplacian matrix defined as
\begin{equation*}
	l_{ij} = \left\{\begin{array}{ll}
		-a_{ij}, & i \neq j \\
		\sum\limits_{i \neq j} a_{ij}, & i=j.
	\end{array} \right.
\end{equation*}
The concentrations of each species are stacked together in the vector $x = [x_{1,1}, \dots x_{1,N}, x_{2,1}, \dots, x_{2,N}]^T \in \mathbb{R}^{2N}$.




\iffalse
Piecewise affine functions are widely used in the modeling of Genetic Regulatory Networks as they remarkably simplify the analysis without compromising excessively the descriptivness of the model [XY].
Under suitable choices of the system parameters we can show that the uncoupled compartments behave indeed like bistable switches, i.e. they have 2 stable equilibria and one unstable equilibria \cite{villani2021global}. 
When using the piecewise affine function we will consider the system under Assumption 1 \textbf{\textcolor{myred}{Will review the calculation below again}}.

\begin{assumption}
	The system's parameters are such that 
	\begin{equation}
		\frac{V_1 V_2}{\delta \gamma_1 \gamma_2} > 1 .
	\end{equation}
\end{assumption}
Assumption 1 guarantees the system to have two stable equilibria $P_{\text{ON}} = (V_1/\gamma_1, (V_1 V_2)/(\gamma_2\gamma_1))$, $P_{\text{OFF}} = (0, 0)$ and an unstable equilibrium $P_{\text{s}} = (\bar{x}_1, \bar{x}_2)$ with 
\begin{equation}
	\begin{split}
		\bar{x}_1 &= \frac{V_1 \theta}{\theta \gamma_1} \left(\frac{V_1 V_2}{\delta \gamma_1 \gamma_2} - 1\right)^{-1}\\
		\bar{x}_2 &= \frac{V_2}{\gamma_2}\bar{x}_1.
	\end{split}
\end{equation}

\fi



\begin{proposition}
	Consider the symmetric laplacian matrix $L$ corresponding to a connected undirected weighted graph. The matrix $L'= L + T$, where $T$ is a nonnegative diagonal matrix with at least one entry strictly greater than zero, is Hurwitz unstable.\
\end{proposition}
\begin{proof} 
	We can write $L = D - A$ where $D$ is the degree matrix and $A$uncunc
	is the adjacency matrix. Applying a congruence transform to $L$ with $D^{-\frac{1}{2}}$ we obtain 
	\begin{equation}
		\tilde{L} = D^{-\frac{1}{2}}(D- A)D^{-\frac{1}{2}} = I - D^{-\frac{1}{2}}AD^{-\frac{1}{2}} = I-B.
		\label{eq:L_congruence}
	\end{equation}
	$L$ has a unique  root equal to 0 and since the congruence transformation preserves the signature of the matrix (number of positive/negative/zero eigenvalues) the transformed matrix $I-B$  has still a unique eigenvalue at 0. 
	Therefore, the matrix $B$ is an irreducible real-nonnegative matrix with single Perron root $\lambda=1$. Using $\Gamma:=\operatorname{diag}(v)$ with $v$ perron eigenvector of $B$ we define the matrix $S = \Gamma^{-1}B \Gamma$. The matrix $S$ is a stochastic matrix \cite[Chapter 2, Theorem 5.4]{berman1994nonnegative}.
	Without loss of generality we can assume that the matrix $T$ has non zero elements only in the first $m$ diagonal entries, therefore we can obtain $L'$ by multiplying $D$ by
	\begin{equation}
		\Sigma = \begin{bmatrix}
			\alpha I_m& 0 \\
			0 & I_{n-m} 
		\end{bmatrix}
	\end{equation}
	with $\alpha >1$ therefore
	\begin{equation}
		L' = D'-A = \Sigma D - A.
	\end{equation}
	Applying a similar congruence transformation to $L'$ we obtain
	\begin{equation}
		\tilde{L'}=I-\Sigma^{\frac{-1}{2}} D^{\frac{-1}{2}} A D^{\frac{-1}{2}} \Sigma^{\frac{-1}{2}}=I-\Sigma^{\frac{-1}{2}} B \Sigma^{\frac{-1}{2}}=I-B^{\prime}.
	\end{equation}
	We can define 
	\begin{equation}
		S^{\prime}:=\Gamma^{-1} B^{\prime} \Gamma=\Gamma^{-1}\left(\Sigma^{\frac{-1}{2}} B \Sigma^{\frac{-1}{2}}\right) \Gamma=\Sigma^{\frac{-1}{2}}\left(\Gamma^{-1} B \Gamma\right) \Sigma^{\frac{-1}{2}}=\Sigma^{\frac{-1}{2}} S \Sigma^{\frac{-1}{2}}.
		`	\end{equation}
	Clearly $S'$ is not stochastic (the first rows do not sum to one while the other rows are untouched) and the first $m$ rows sums are less than one. Therefore, by Lemma \ref{lm:substochastic} we can conclude that the spectral radius of $S'$ is strictly less than one. As $S'$ and $B'$ share the same set of eigenvalues, this allows us to conclude that the matrix $B'$ has spectral radius strictly less than one. It therefore follows that the matrix $L'$ has at least one eigenvalue with positive real part, therefore it is Hurwitz unstable.
\end{proof}
Proposition \ref{prop:main_result_ccw_domain} proves that for a complete analysis of the dynamics in \eqref{eq:bistable_network_og} it is sufficient to analyze the equilibria in the saturated domain as they are the only (locally) stable equilibria for the dynamics. Furthermore, the calculation of equilibria in saturated domains is pretty straightforward as the matrix $M_\alpha$ is the same for all saturated domains. For certain graph topologies, as we previously showed, it is possible to compute the minimum coupling gain to ensure the existence of only synchronized equilibria in the saturated domains.


\begin{lemma}
	\label{lm:substochastic}
	Consider an irreducible nonnegative  matrix $M\in \mathbb{R}^{n \times n}$ whose rows sum is one for all rows, except for the first $m$ rows whose sum is equal to $r$, with $r<1$ (or $r>1$). The spectral radius of $M$ is respectively strictly less than one (or strictly greater than one).
\end{lemma}
\begin{proof}
	As $M$ is an irreducible nonnegative matrix, Perron-Frobenius theory guarantees the existence of the eigenvalue-eigenvector pair $(\lambda, v)$ with $\lambda=\rho(M)$ and $v>0$. Without loss of generality we can assume $||v||_1=1$. The following equality will be useful later
	\begin{equation}
		\begin{aligned}
			|\lambda| &=\|\lambda v\|_{1} \\
			&=\|v A\|_{1} \\
			&=\sum_{j} \sum_{k} v_{j} A_{j k}
		\end{aligned}.
		\label{eq:perron_sum}
	\end{equation}
	Define
	\begin{equation}
		\epsilon_j \vcentcolon= \frac{1}{n}(1- \sum\limits_{k=1}^n A_{jk})
	\end{equation}
	and consider $\epsilon$ the vector containing all the $\epsilon_j$ entries. Notice that in case $r<1$ ($r>1$), the first $m$ entries of $\epsilon$ are strictly positive (strictly negative), while the remaining $n-m$ entries are zero. Summing $\epsilon_j$ to all the entries in each row $j$ defines a stochastic matrix $\tilde{A} = A+\epsilon^{T} \mathbf{1}$. From \eqref{eq:perron_sum}
	\begin{equation}
		\begin{aligned}
			|\lambda| &=\sum_{j} \sum_{k} v_{j}\left(A_{j k}+\epsilon_{j}-\epsilon_{j}\right) \\
			&=\sum_{j} \sum_{k} v_{j}\left(A_{j k}+\epsilon_{j}\right)-\sum_{j} \sum_{k} v_{j} \epsilon_{j} \\
			&=\left\|v\left(A+\epsilon^{T} \mathbf{1}\right)\right\|_{1}-n(\boldsymbol{\epsilon} \cdot v)
		\end{aligned}
	\end{equation}
	and therefore
	\begin{equation}
		\begin{aligned}
			|\lambda| &=\|v \tilde{A}\|_{1}-n(\epsilon \cdot v) \\
			&=1-n(\epsilon \cdot v) 
		\end{aligned}
	\end{equation}
	Therefore, we can conclude that if $r<1$, the spectral radius is strictly smaller than one while for $r>1$, the spectral radius is strictly greater than one.
	
\end{proof}




















The concentrations of each species can be stacked together in the vectors  $x_1 = [x_{1,1}, \dots, x_{1,N}]^T$ and $x_2 = [x_{2,1}, \dots, x_{2,N}]^T$
so that we rewrite \eqref{eq:bistable_network_og_repeated} in vectorized form 

\begin{equation}
	\begin{aligned}
		&\dot{x}_{1}=-(\Gamma_{1} + L) x_{1}+V_{1} g\left(x_{2}\right) \\
		&\dot{x}_{2}=-\Gamma_{2} x_{2}+V_{2} x_{1}
	\end{aligned}
	\label{eq:bistable_network_vector}
\end{equation}
where the matrix $L = [l_{ij}]$ is the symmetric Laplacian matrix defined as
\begin{equation*}
	l_{ij} = \left\{\begin{array}{ll}
		-a_{ij}, & i \neq j \\
		\sum\limits_{i \neq j} a_{ij}, & i=j.
	\end{array} \right.
\end{equation*}
and $g(x_2)=[g(x_{2,1}), \dots, g(x_{2,N})]^T$.
We can restrict the dynamics to the set  
\begin{equation*}
	\mathcal{B}:= \displaystyle\prod_{k=1}^{N} \left[0, \frac{V_1}{\gamma_1}\right] \displaystyle\prod_{k=1}^{N} \left[0, \frac{V_2 V_1}{\gamma_2 \gamma_1}\right], 
	\label{eq:domain_definition}
\end{equation*}
as it can be shown that is forward invariant.
The phase space $\mathcal{B}$, can be partitioned into different \textit{domains} such that the restriction of the vector field in \eqref{eq:bistable_network_og_repeated} is affine on each domain. 
\begin{definition} Let  $\mathcal{T} \subset \mathbb{R}^{N}$ denote the set of $N$ dimensional vectors with entries in $\{-1, 0, +1\}$. We can associate each element $\alpha$ in $\mathcal{T}$ to a \textit{domain} $\Omega_{\alpha}$ defined as
	\begin{equation*}
		\begin{aligned}
			\Omega_{\alpha}:=\left\{x\in\right. \mathcal{B} \mid &x_{2, j} \geq \theta + \delta,\text{ if } \alpha_{j}=1 \\
			&x_{2, j} \leq \theta,\text{ if } \alpha_{j}=-1 \\
			\theta<&x_{2, j}<\theta + \delta,\ \left.\text{if }\alpha_{j}=0\right\}.
		\end{aligned}
		\label{eq:def_omega}
	\end{equation*}
	A domain $\Omega_{\alpha}$ is called \textit{saturated} if $\alpha \in \Lambda_{e} :=\{\alpha \in \mathcal{T}: \alpha_{i, j} \in \{-1, 1\}\}$, \textit{interior} if $\alpha \in \Lambda_0 :=\{\alpha \in \mathcal{T}: \alpha_{i, j} = 0\}$ and \textit{mixed} if $\alpha \in \Lambda_m := \mathcal{T}/\left(\Lambda_0 \cup \Lambda_e \right)$.
\end{definition}
The proposed definition of domains $\Omega_{\alpha}$ defines indeed a partition of $\mathcal{B}$ since it can be easily verified that $\mathcal{B} = \cup_{\alpha \in \mathcal{T}}\Omega_{\alpha}$ and $\Omega_{\alpha} \cap \Omega_{\alpha'} = \emptyset$ when $\alpha \neq \alpha '$. 




==> extras.tex <==
	\paragraph{Analysis of uncoupled compartment}
The next step of the proof consists in showing that under the assumption (Assumption 3) that all equilibria of the uncoupled compartment are isolated and that all trajectories of the uncoupled compartment converge toward one equilibrium. Consider the autonomous vector field in \eqref{eq:autonomous_limit}. Then, the function 
\begin{equation}
	E(x)=-1/2 G(x)^TA G(x) +  \sum_{i=1}^{2} \int_{0}^{g_i(x_i)} \gamma_{i}\ g_i^{-1}(\tau) \operatorname{d} \tau
	\label{eq:energy_function_general}
\end{equation} is monotone nonincreasing along the flow of \eqref{eq:autonomous_limit}. The proof is divided into two parts. In the first part we will show that the directional derivative of $E(x)$, along the vector flow $h(x)$ is non positive, at all points where $E(x)$ is differentiable. In the second part, we complete the proof by computing $E^o(x, h(x))$ - the generalized directional derivative of $E$, along $h(x)$ - at the points where $E(x)$ is not differentiable.\\ 
\textbf{Part 1).} For all $x$ where $E(x)$ is differentiable,  we can compute the standard directional derivative of $E(x)$ along the vector flow $h(x)$ (Lie derivative $\mathcal{L}_{h(x)} E(x)$. We start by computing 
\begin{equation}
	\nabla E(x)=\frac{\partial}{\partial x} E(x)= - \frac{1}{2} \sum\limits_{i=1}^{2}  \sum_{j=1}^{2} a_{ij}\frac{\partial }{\partial x}\left(g_i(x) g_j(x)\right)+ \sum_{i=1}^{2}\frac{\partial }{\partial x}\int_{0}^{g_i(x)} \gamma_{i}g_i^{-1}(\tau) \operatorname{d} \tau =
\end{equation}
%\begin{equation}
%	=- \frac{1}{2} \sum\limits_{i=1}^{2N}  \sum_{j=1}^{2N} a_{ij}\left(\frac{\operatorname{d}}{\operatorname{d}t}G_i(x) G_j(x) + G_i(x)\frac{\operatorname{d}}{\operatorname{d}t} G_j(x) \right) + \sum_{i=1}^{2N} \frac{\partial}{\partial x_i}G_i(x) \Gamma_{i}x_i =
%\end{equation}


\begin{equation}
	=- \frac{1}{2} \sum\limits_{i=1}^{2}  \sum_{j=1}^{2} a_{ij}\left(\frac{\partial}{\partial x}g_i(x)  g_j(x) + g_i(x)\frac{\partial}{\partial x}g_j(x) \right) + \sum_{i=1}^{2}\frac{\partial}{\partial x}g_i(x) \gamma_{i}x_i =
\end{equation}
%}\frac{\partial}}{\partial x_i}G_i(x) 
Since the matrix $A$ is symmetric,

\begin{equation}
=- \sum\limits_{i=1}^{2}  \sum_{j=1}^{2} a_{ij}\frac{\partial}{\partial x}g_i(x) g_j(x) + \sum_{i=1}^{2}\frac{\partial}{\partial x}g_i(x) \gamma_{i}x_i =
\end{equation}
and therefore
\begin{equation}
=- \sum\limits_{i=1}^{2} \frac{\partial}{\partial x}g_i(x)  \left(\sum_{j=1}^{2} a_{ij} g_j(x)  -\gamma_{i}x_i  .
\right)\end{equation} 
Since  $h(x)=\sum_{j=1}^{2} a_{ij} g_j(x)  -\gamma_{i}x_i  $, and $G(x)$ is a diagonal nonlinearity, i.e. each of its entries depends only on the corresponding species, we can rewrite 
\begin{equation}
\nabla E(x)= \frac{\partial E}{\partial x}	=-\frac{\partial }{\partial x} G(x) h(x)
\label{eq:gradient_calc}
\end{equation} 
and therefore

\begin{equation}
\mathcal{L}_{h(x)} E(x) =\frac{\partial E}{\partial x}^T h(x) = - h(x)^T \frac{\partial }{\partial x} G(x) h(x)  \leq 0
\end{equation}
as $\frac{\partial}{\partial x}G(x)$ is a positive semidefinite matrix under Assumption 2.
\\
\textbf{Part 2)} Consider a generic point $\hat{x} = [\hat{x}^1, \hat{x}^2]^T$ where the energy function $E(x)$ is not differentiable. This implies that either $g_1(x)$, $g_2(x)$, or both are not differentiable in $\hat{x}$ with respect to $x$.  In this point, $	E^o(\hat{x}, h(\hat{x}))$, the generalized directional derivative of $E(x)$ along the vector field $h(x)$ is defined as
\begin{equation}
E^o(\hat{x}, h(\hat{x}))=\max \{\langle\xi, h(\hat{x})\rangle, \quad \xi \in \partial E(\hat{x})\}. \\
\end{equation}
where $\partial E(\hat{x})$ is the generalized gradient of $E(x)$, defined as
\begin{equation}
\partial E(\hat{x})=\overline{\operatorname{co}}\left\{\lim \nabla E(x): x_i \rightarrow \hat{x}\right\}.
\end{equation}
$\partial E(\hat{x})$ is the closed convex hull of the sets of all possible $\lim\limits_{ x_i \rightarrow \hat{x}} \nabla E(x)$ when we consider all sequences $x_i$ converging to $\hat{x}$ such that $E(x)$ is
differentiable at $x_i$ and the indicated limit exists \cite{clarke1975generalized}. Let's assume that both $g_1(x)$ and $g_2(x)$ are not differentiable in $\hat{x}$. In the case only one of the function is non differentiable, the argument is analogous.  Without loss of generality, we can restrict the  analysis to a arbitrarily small neighborhood $B_\epsilon(\hat{x})$ of $\hat{x}$. In this neighbourhood, the energy function $E(x)$ is not differentiable in all points where either $x_1=\hat{x}_1$ or $x_2=\hat{x}_2$. Therefore, the gradient of the function $E(x)$ is  well defined on all points in $
\Omega = \left((\hat{x}^1-\epsilon, \hat{x}^1)\cup(\hat{x}^1, \hat{x}^1+\epsilon)\right)
\times
\left((\hat{x}^2-\epsilon, \hat{x}^2)\cup(\hat{x}^2, \hat{x}^2+\epsilon)\right)$. The set $\Omega$ is composed by 4 open, disjoint sets on which $\nabla E(x)$ is well defined. Let's call these domains $D_1=(\hat{x}^1, \hat{x}^1+\epsilon)\times (\hat{x}^2, \hat{x}^2+\epsilon)$, $D_2=(\hat{x}^1-\epsilon, \hat{x}^1)\times (\hat{x}^2, \hat{x}^2+\epsilon$, $D_3=(\hat{x}^1-\epsilon, \hat{x}^1)\times (\hat{x}^2- \epsilon, \hat{x}^2)$, and $D_4=(\hat{x}^1, \hat{x}^1+\epsilon) \times (\hat{x}^2- \epsilon, \hat{x}^2)$. Now, consider a sequence ${x_i}$ that is ultimately contained in only one of these domains, e.g. $D_1$.  For each $x_i$, as previously computed in \eqref{eq:gradient_calc}, $\nabla E(x_i) = - \frac{\partial}{\partial x}G(x_i)h(x_i)$ and its limit is  equal to $-\operatorname{diag}\{\lim\limits_{x_i^1\to \hat{x}_i^{1^+}}\frac{\partial }{\partial x_1}g_1(x_1), \lim\limits_{x_i^2\to \hat{x}_i^{2^+}}\frac{\partial }{\partial x_2}g_2(x_2)\} h(\hat{x}):= \nabla_{D_1} E(x)$. One can analogously define $ \nabla_{D_2} E(\hat{x})$, $ \nabla_{D_3} E(\hat{x})$, $ \nabla_{D_4} E(\hat{x})$ and therefore prove that 
\begin{equation}
\partial E(x) = \overline{\operatorname{co}}\{\nabla_{D_1} E(\hat{x}), \nabla_{D_2} E(\hat{x}),  \nabla_{D_3} E(\hat{x}),  \nabla_{D_4} E(\hat{x})\}.
\label{eq:gradient_generalized_set}
\end{equation} 
Indeed, for sequences that are not ultimately contained in only one domain, there will be no additional values for the corresponding limit. If a sequence does not stay within a single domain and instead alternates or oscillates among multiple domains, it won't have a unique limit, unless the limit for each subsequence contained in the single domains are equal.  In this case, the same limit  is already accounted for in the set of possible limit values, $\partial E(x)$, as in  \eqref{eq:gradient_generalized_set}. 
Finally, the closed convex hull  in \eqref{eq:gradient_generalized_set} is obtained as:
\begin{equation}
\begin{array}{r}
\partial E(x)= \overline{\operatorname{co}}\{\nabla_{D_1} E(\hat{x}), \nabla_{D_2} E(\hat{x}),  \nabla_{D_3} E(\hat{x}),  \nabla_{D_4} E(\hat{x})\}. \\
=\left\{\sum_{i=1}^4\lambda_i \nabla_{D_i} E(\hat{x}), \sum_{i=1}^4 \lambda_i=1 \text { and } \lambda_i \geq 0\right\}
\end{array}
\end{equation}
The generalized directional derivative $E^o(x, h(\hat{x}))$ evaluated in $\hat{x}$ where $E$ is not differentiable is defined as 
\begin{equation}
\begin{array}{r}
E^o(\hat{x}, h(\hat{x}))=\max \{\langle\xi, h(\hat{x})\rangle, \quad \xi \in \partial E(\hat{x})\}. \\
= \max\left\{\langle\sum_{i=1}^4\lambda_i \nabla_{D_i} E(\hat{x}), h(\hat{x})\rangle,\ \sum_{i=1}^4 \lambda_i=1, \ \lambda_i \geq 0\right\} \leq 0. \\
= \max\{\langle \nabla_{D_i} E(\hat{x}), h(\hat{x})\rangle,\ i=1, 2, 3, 4\}
\end{array}
\label{eq:generalized_lie_derivative}
\end{equation}
Therefore, $E^o(x, h(x))\leq 0$ for all $x$ in the state space and we can conclude that the energy function $E^o(x, h(x))$ is non-increasing along the forward trajectories of the system in  \eqref{eq:autonomous_limit}.
\paragraph{Lasalle's Analysis }
According to Theorem \ref{thm:lasalle_nonsmooth} all trajectories converge to the largest invaraint set in $\mathcal{S}=\left\{x \in \mathcal{B}: E^o(x, h(x))=0\right\}$. In the following we show that this set is the set of equilibria. The set $\mathcal{S}$ is the union of three different components:
\begin{itemize}
\item $ \mathcal{S}_{\text{eq}} = \{x:\ h(x)=0\}$, the set of equilibrium points;

\item $	\mathcal{S}_{\text{sat}} = \overline{\{x\in \mathcal{S}: \frac{\partial}{\partial x_1}g_1(x_1)= 0 \land \frac{\partial}{\partial x_2}g_2(x_2)=0 \}}$\footnote{\label{note1} We consider the closure of the set, including boundary points where $g_i$ are not differentiable, but the corresponding generalized derivative remains zero.},  the set of points where both activation functions are constant;

\item  $\mathcal{S}_{\text{mix}} = \overline{\{x\in \mathcal{S}: \frac{\partial}{\partial x_1}g_1(x_1) \frac{\partial}{\partial x_2}g_2(x_2)=0,\  \frac{\partial}{\partial x_1}g_1(x_1) \neq\frac{\partial}{\partial x_2}g_2(x_2) \}}$, the set of points where only one of the activation functions is constant.
\end{itemize}
A simplified, intuitive visualization of the sets $\mathcal{S}{\text{eq}}, \mathcal{S}{\text{sat}}, \mathcal{S}_{\text{mix}}$ can be seen in Figure \ref{fig:domain_example}. $\mathcal{S}_{\text{eq}} \subset \mathcal{M}$ as equilibria are clearly invariant. We proceed to demonstrate that in both $\mathcal{S}_{\text{sat}}$ and $\mathcal{S}_{\text{mix}}$, the only invariant sets are the equilibria. The proof for $\mathcal{S}_{\text{sat}}$ is presented here, as the proof for $\mathcal{S}_{\text{mix}}$ follows a similar logic.

The set $\mathcal{S}_{\text{sat}}$ can be obtained as the disjoint union of sets of the form $[a_i^1, b_i^1] \times [a_i^2, b_i^2]$ where $a_i^1 \leq b_i^1$ and $a_i^2 \leq b_i^2$. 
\begin{equation}
\mathcal{S}_{\text{sat}} = \bigcup\limits_{i}\ [a_i^1, b_i^1] \times [a_i^2, b_i^2]
\end{equation}
The dynamics, restricted to each of these sets $\ [a_i^1, b_i^1] \times [a_i^2, b_i^2]$ has the form
\begin{equation}
\begin{aligned}
\dot{x}_1 = -\gamma_{1} x_1 +c_1 \\
\dot{x}_2 = -\gamma_{2}x_2 +c_2 
\end{aligned}.
\label{eq:pwa_restriced_sat}
\end{equation}
Assume $x^* = [x^*_1, x^*_2]\in [a_i^1, b_i^1] \times [a_i^2, b_i^2]$ is not an equilibrium, then there exists $\tilde{t} \in$ $(-\infty,+\infty)$ such that \textcolor{black}{$\phi\left(\tilde{t}, x^*\right) \notin [a_i^1, b_i^1] \times [a_i^2, b_i^2]$} and $\phi\left(\tilde{t}, x^*\right) \notin \mathcal{S}_{\text{sat}}$ as the only invariant set under the dynamics in \eqref{eq:pwa_restriced_sat} in $[a_i^1, b_i^1] \times [a_i^2, b_i^2]$ is the set of equilibria.




\begin{figure}
\centering
\includegraphics[width=0.95\linewidth]{domain_representation}
\caption{Graphical visualization of the sets $\mathcal{S}_{\text{eq}}, \mathcal{S}_{\text{sat}}, \mathcal{S}_{\text{mix}}$ for a bistable system like \eqref{eq:autonomous_limit} where both $g_1$ and $g_2$ are piecewise affine functions.}
\label{fig:domain_example}
\end{figure}




%\begin{equation}
%	\mathcal{S}_{p\text{eq}} = \{x\in \mathcal{S}: h_1(x)\neq 0 \lor  h_2(x)\neq 0 \}
%\end{equation}
%	, i.e. the set of non equilibrium points where the generalized directional dertivative of the energy function $E^o(x, h(x))$ along the vector field $h(x)$ is zero. 


\iffalse
$$
\mathcal{S}=\left(\cup_{\alpha \in \Lambda_e} \Omega_\alpha\right) \cup\left(\cup_{\alpha \in \Lambda^m} I_\alpha\right) \cup \mathcal{E}_0
$$
where:
\begin{itemize}
\item $\cup_{\alpha \in \Lambda_c} \Omega_\alpha$ is the union of all saturated regions. Indeed, for all $x \in \cup_{\alpha \in \Lambda_e} \Omega_\alpha$, no species $x_{i, j}$ is in the linear region, therefore according to (24) $E^o(x, F(x))=$ $0, \forall x \in \cup_{\alpha \in \Lambda_e} \Omega_\alpha$.
\item $\cup_{\alpha \in \Lambda_m} I_\alpha$ is the union (by definition), over all the mixed regions, of the subsets $I_\alpha$ where the components of the vector field corresponding to the species in the linear region vanish. Therefore the sum in (24) has all terms equal to zero.
\item $\mathcal{E}_0$ is the set of equilibria in the linear region. Indeed, the only points in the interior domain such that $E^o(x ; F(x))=0$ are the equilibria (the square of all the entries of the vector field $F(x)$ has to be zero).
\end{itemize}

\fi
We proved that all trajectories of the limiting autonomous vector field \eqref{eq:autonomous_limit} converge to the set of equilibria. Furthermore, the existence of the energy function in \eqref{eq:energy_function_general} guarantees that no equilibria are chained cyclically. Finally as all the equilibria of the uncoupled compartment are isolated (Assumption 3) we can conclude that for all forward trajectories that synchronize, every compartment converges to the same equilibrium point $P$. Notably, this point $P$ is also an equilibrium of the isolated compartment (Corollary \ref{corollary_main_equilibria}, Appendix C).
\end{proof}




\subsection{Synchronization Conditions}
\begin{proposition}
Consider the networked system in \eqref{eq:bistable_network_og} under Assumption 1, 2, and 3. Then, there exists a minimum value $\lambda^*$ such that,	 when the algebraic connectivity $\lambda$ of the laplacian $L_1$ is greater than $\lambda^*$, the networked system in \eqref{eq:bistable_network_og} synchronizes. 
\end{proposition}
\begin{proof}
Each bistable switch can be modeled as a compartment made up of 4 cyclically interconnected subsystems $H_{1,j}$, $H_{2,j}$, $H_{3,j}$, $H_{4,j}$  
\begin{equation}
\begin{aligned}
H_{1,j} &: \left\{\begin{array}{ll}
	\dot{x}_{1,j} =- \gamma_1 x_{1,j}  + v_{1,j} \\
	y_{1,j} = x_{1,j}
\end{array}\right. \\
H_{2,j} &: \left\{\begin{array}{ll}
	y_{2,j}= g_1(v_{2,j})
\end{array}\right. \\
H_{3,j} &: \left\{\begin{array}{ll}
	\dot{x}_2 =- \gamma_2 x_{2,j}  + v_{3,j} \\
	y_{3,j} = x_{2,j}
\end{array}\right. \\
H_{4,j} &: \left\{\begin{array}{ll}
	y_{4,j} = g_2(v_{3,j})
\end{array}\right. .
\end{aligned}
\label{eq:I_O_compartments}
\end{equation}
where $\gamma_{1}, \gamma_{2}>0$ and the functions $g_1$ and $g_2$  satisfy Assumption 2.
The interconnections are encompassed by the inputs
\begin{equation}
v_{k, j}=u_{k, j}+\sum_{z=1}^{n} a_{j, z}^{k}\left(x_{k, z}-x_{k, j}\right)
\label{eq:compartment_inputs}
\end{equation}
where $u_{1,j}=V_1 y_{4,j}$, $u_{2,j}=y_{1,j}$, $u_{3,j}=V_2y_{1,j}$, and $u_{4,j}=y_{3,j}$ where the second term in \eqref{eq:compartment_inputs} represents the diffusion among the compartments.  For the rest of this section we assume the diffusion involving only the first species, therefore $a^2_{j,z}=a^3_{j,z}=a^4_{j,z}=0$.
Such a coupling scheme corresponds to the cyclic interconnection matrix
\begin{equation}
\Sigma_g = \begin{bmatrix}
0 & 0 & 0& V_1 \\
1 & 0 & 0 & 0\\
0 & 1 & 0 & 0\\
0 & 0 & V_2 & 0
\end{bmatrix}.
\end{equation}
\end{proof}




\begin{figure}
\centering
\includegraphics[width=0.95\linewidth]{cocoercivity_diagram}
\caption{Input-output scheme representing the mathemtical model in \eqref{eq:I_O_compartments}. }
\label{fig:cocoercivitydiagram}
\end{figure}

The operator $H_{1,j}$  and $H_{3,j}$ can be associated to I/O cocoercive operators with constants respectively $\alpha_1 = \gamma_1$ and $\alpha_3=\gamma_3$. The I/O operator $H_{2,j}$ and $H_{4,j}$ are also relaxed cocoercive with constant $\alpha_2=1/\ell_1$ and $\alpha_4=1/\ell_2$ where $\ell_1$ and $\ell_2$ are the Lipschitz constant for the static nonlinearities $g_1$ and $g_2$ respectively  \cite{scardovi2010synchronization} .


We can finally formulate the synchronization problem in terms of the diagonal stability of the dissipation matrix \eqref{eq:dissipativity_2d} as in \cite{scardovi2010synchronization}. 
\begin{equation}
E = \begin{bmatrix}
-(\gamma_1+\lambda) & 0 & V_1 \\
1 &  -1/\ell_1 & 0 &0 \\
0 & 1 & -\gamma_2 & 0 \\
0 & 0 & V_2 & -1/\ell_2
\label{eq:dissipativity_2d}
\end{bmatrix}.
\end{equation}
where $\lambda$ is the algebraic connectivity corresponding to the undirected laplacian matrix representing the diffusion terms between the first species. By Proposition \ref{prop:positive_loop_diagonal_stability} in Appendix A the matrix $E$ in \eqref{eq:dissipativity_2d} is diagonally stable if and only if
\begin{equation}
\frac{V_1 V_2 \ell_1 \ell_2}{(\gamma_{1}+\lambda)\gamma_2} < 1,
\end{equation}
that is if 
\begin{equation}
\lambda > \frac{V_1 V_2 \ell_1 \ell_2}{\gamma_2} - \gamma_1 =\lambda^*.
\end{equation}

Therefore, we can conclude that an undirected, connected  graph with algebaic connectivity $\lambda > \lambda^*$ guarantees global synchronization for the networked system in \eqref{eq:bistable_network_og}. \\

\subsection{Omega limit sets analysis}

In this first part of the analysis, the focus is on characterizing the omega limit set of a network that achives global synchronization. The primary result is outlined in Theorem \ref{thm:chain_recurrence_synchronization}.


\begin{thm}
Consider the networked system in \eqref{eq:bistable_network_og} under  Assumption 1 and 2, and further assume that all solutions of the networked system in \eqref{eq:bistable_network_og} synchronize. Then, each compartment converges towards one of the equilibria of the uncoupled compartment. 
\label{thm:chain_recurrence_synchronization}
\end{thm}



\begin{proof}
From the point of view of the single i-th compartment, the dynamics writes as follows
\begin{equation}
\begin{aligned}
& \dot{x}_{1, i}=-\gamma_1 x_{1, i}+V_1 g_2(x_{2,i})+d^1_i(t) \\
& \dot{x}_{2, i}=-\gamma_2 x_{2, i}+V_2 g_1(x_{1,i}) %+d^2_i(t) .
\end{aligned}
\label{eq:networked_system_time_1}
\end{equation}
with $d_i^(t) = \sum_{j} a_{ij}^1\left(x_{1, j}-x_{1, i}\right)$. 
For each initial condition{ $\mathbf{x(0)}$,} we can consider the signals $d_i(t)$ as purely time dependent so that we can write the dynamics of the \textit{i-th} compartment in \eqref{eq:networked_system_time_1} as a nonautonomous system
\begin{equation}
\dot{x}_i(t)  = -\Gamma x_i + A G(x_i) + [d_i^1(t)\ \ 0]^T:= f_i(x_i, t) 
\label{eq:nonautonomous_general}
\end{equation}
where  $x_i=[x_{1,i}, x_{2,i}]^T$.  The autonomous system
\begin{equation}
\dot{z}_i(t) = -\Gamma z_i + A G(z_i) := h(z_i).
\label{eq:autonomous_limit}
\end{equation}
is the limiting vector field in \eqref{eq:nonautonomous_general} under the condition $d_i^1(t)=0$.
As the difference between the two functions in \eqref{eq:nonautonomous_general}, \eqref{eq:autonomous_limit}
\begin{equation}
f_i(x_i, t) - h(x_i) =  [d_i^1(t)\ \ 0]^T
\end{equation}
does not depend on the state $x_i$,  $f_i(x_i, t)$ uniformly converges to $h(x_i)$ for every compact set in $\mathbb{R}^n$.  Therefore, under the synchronization assumption, the non-autonomous system in \eqref{eq:networked_system_time_1}  is asymptotically autonomous with limit equation \eqref{eq:autonomous_limit}.  
\paragraph{Analysis of uncoupled compartment}
The next step of the proof consists in showing that all equilibria of the uncoupled compartment are isolated and that all trajectories of the uncoupled compartment converge toward one equilibrium. Consider the autonomous vector field in \eqref{eq:autonomous_limit}. Then, the function 
\begin{equation}
E(x)=-1/2 G(x)^TA G(x) +  \sum_{i=1}^{2} \int_{0}^{g_i(x_i)} \gamma_{i}\ g_i^{-1}(\tau) \operatorname{d} \tau
\label{eq:energy_function_general}
\end{equation} is monotone nonincreasing along the flow of \eqref{eq:autonomous_limit}. The proof is divided into two parts. In the first part we will show that the directional derivative of $E(x)$, along the vector flow $h(x)$ is non positive, at all points where $E(x)$ is differentiable. In the second part, we complete the proof by computing $E^o(x, h(x))$ - the generalized directional derivative of $E$, along $h(x)$ - at the points where $E(x)$ is not differentiable.\\ 
\textbf{Part 1).} For all $x$ where $E(x)$ is differentiable,  we can compute the standard directional derivative of $E(x)$ along the vector flow $h(x)$ (Lie derivative $\mathcal{L}_{h(x)} E(x)$. We start by computing 
\begin{equation}
\nabla E(x)=\frac{\partial}{\partial x} E(x)= - \frac{1}{2} \sum\limits_{i=1}^{2}  \sum_{j=1}^{2} a_{ij}\frac{\partial }{\partial x}\left(g_i(x) g_j(x)\right)+ \sum_{i=1}^{2}\frac{\partial }{\partial x}\int_{0}^{g_i(x)} \gamma_{i}g_i^{-1}(\tau) \operatorname{d} \tau =
\end{equation}
%\begin{equation}
%	=- \frac{1}{2} \sum\limits_{i=1}^{2N}  \sum_{j=1}^{2N} a_{ij}\left(\frac{\operatorname{d}}{\operatorname{d}t}G_i(x) G_j(x) + G_i(x)\frac{\operatorname{d}}{\operatorname{d}t} G_j(x) \right) + \sum_{i=1}^{2N} \frac{\partial}{\partial x_i}G_i(x) \Gamma_{i}x_i =
%\end{equation}


\begin{equation}
=- \frac{1}{2} \sum\limits_{i=1}^{2}  \sum_{j=1}^{2} a_{ij}\left(\frac{\partial}{\partial x}g_i(x)  g_j(x) + g_i(x)\frac{\partial}{\partial x}g_j(x) \right) + \sum_{i=1}^{2}\frac{\partial}{\partial x}g_i(x) \gamma_{i}x_i =
\end{equation}
%}\frac{\partial}}{\partial x_i}G_i(x) 
Since the matrix $A$ is symmetric,

\begin{equation}
=- \sum\limits_{i=1}^{2}  \sum_{j=1}^{2} a_{ij}\frac{\partial}{\partial x}g_i(x) g_j(x) + \sum_{i=1}^{2}\frac{\partial}{\partial x}g_i(x) \gamma_{i}x_i =
\end{equation}
and therefore
\begin{equation}
=- \sum\limits_{i=1}^{2} \frac{\partial}{\partial x}g_i(x)  \left(\sum_{j=1}^{2} a_{ij} g_j(x)  -\gamma_{i}x_i  .
\right)\end{equation} 
Since  $h(x)=\sum_{j=1}^{2} a_{ij} g_j(x)  -\gamma_{i}x_i  $, and $G(x)$ is a diagonal nonlinearity, i.e. each of its entries depends only on the corresponding species, we can rewrite 
\begin{equation}
\nabla E(x)= \frac{\partial E}{\partial x}	=-\frac{\partial }{\partial x} G(x) h(x)
\label{eq:gradient_calc}
\end{equation} 
and therefore

\begin{equation}
\mathcal{L}_{h(x)} E(x) =\frac{\partial E}{\partial x}^T h(x) = - h(x)^T \frac{\partial }{\partial x} G(x) h(x)  \leq 0
\end{equation}
as $\frac{\partial}{\partial x}G(x)$ is a positive semidefinite matrix under Assumption 2.
\\
\textbf{Part 2)} Consider a generic point $\hat{x} = [\hat{x}^1, \hat{x}^2]^T$ where the energy function $E(x)$ is not differentiable. This implies that either $g_1(x)$, $g_2(x)$, or both are not differentiable in $\hat{x}$ with respect to $x$.  In this point, $	E^o(\hat{x}, h(\hat{x}))$, the generalized directional derivative of $E(x)$ along the vector field $h(x)$ is defined as
\begin{equation}
E^o(\hat{x}, h(\hat{x}))=\max \{\langle\xi, h(\hat{x})\rangle, \quad \xi \in \partial E(\hat{x})\}. \\
\end{equation}
where $\partial E(\hat{x})$ is the generalized gradient of $E(x)$, defined as
\begin{equation}
\partial E(\hat{x})=\overline{\operatorname{co}}\left\{\lim \nabla E(x): x_i \rightarrow \hat{x}\right\}.
\end{equation}
$\partial E(\hat{x})$ is the closed convex hull of the sets of all possible $\lim\limits_{ x_i \rightarrow \hat{x}} \nabla E(x)$ when we consider all sequences $x_i$ converging to $\hat{x}$ such that $E(x)$ is
differentiable at $x_i$ and the indicated limit exists \cite{clarke1975generalized}. Let's assume that both $g_1(x)$ and $g_2(x)$ are not differentiable in $\hat{x}$. In the case only one of the function is non differentiable, the argument is analogous.  Without loss of generality, we can restrict the  analysis to a arbitrarily small neighborhood $B_\epsilon(\hat{x})$ of $\hat{x}$. In this neighbourhood, the energy function $E(x)$ is not differentiable in all points where either $x_1=\hat{x}_1$ or $x_2=\hat{x}_2$. Therefore, the gradient of the function $E(x)$ is  well defined on all points in $
\Omega = \left((\hat{x}^1-\epsilon, \hat{x}^1)\cup(\hat{x}^1, \hat{x}^1+\epsilon)\right)
\times
\left((\hat{x}^2-\epsilon, \hat{x}^2)\cup(\hat{x}^2, \hat{x}^2+\epsilon)\right)$. The set $\Omega$ is composed by 4 open, disjoint sets on which $\nabla E(x)$ is well defined. Let's call these domains $D_1=(\hat{x}^1, \hat{x}^1+\epsilon)\times (\hat{x}^2, \hat{x}^2+\epsilon)$, $D_2=(\hat{x}^1-\epsilon, \hat{x}^1)\times (\hat{x}^2, \hat{x}^2+\epsilon$, $D_3=(\hat{x}^1-\epsilon, \hat{x}^1)\times (\hat{x}^2- \epsilon, \hat{x}^2)$, and $D_4=(\hat{x}^1, \hat{x}^1+\epsilon) \times (\hat{x}^2- \epsilon, \hat{x}^2)$. Now, consider a sequence ${x_i}$ that is ultimately contained in only one of these domains, e.g. $D_1$.  For each $x_i$, as previously computed in \eqref{eq:gradient_calc}, $\nabla E(x_i) = - \frac{\partial}{\partial x}G(x_i)h(x_i)$ and its limit is  equal to $-\operatorname{diag}\{\lim\limits_{x_i^1\to \hat{x}_i^{1^+}}\frac{\partial }{\partial x_1}g_1(x_1), \lim\limits_{x_i^2\to \hat{x}_i^{2^+}}\frac{\partial }{\partial x_2}g_2(x_2)\} h(\hat{x}):= \nabla_{D_1} E(x)$. One can analogously define $ \nabla_{D_2} E(\hat{x})$, $ \nabla_{D_3} E(\hat{x})$, $ \nabla_{D_4} E(\hat{x})$ and therefore prove that 
\begin{equation}
\partial E(x) = \overline{\operatorname{co}}\{\nabla_{D_1} E(\hat{x}), \nabla_{D_2} E(\hat{x}),  \nabla_{D_3} E(\hat{x}),  \nabla_{D_4} E(\hat{x})\}.
\label{eq:gradient_generalized_set}
\end{equation} 
Indeed, for sequences that are not ultimately contained in only one domain, there will be no additional values for the corresponding limit. If a sequence does not stay within a single domain and instead alternates or oscillates among multiple domains, it won't have a unique limit, unless the limit for each subsequence contained in the single domains are equal.  In this case, the same limit  is already accounted for in the set of possible limit values, $\partial E(x)$, as in  \eqref{eq:gradient_generalized_set}. 
Finally, the closed convex hull  in \eqref{eq:gradient_generalized_set} is obtained as:
\begin{equation}
\begin{array}{r}
\partial E(x)= \overline{\operatorname{co}}\{\nabla_{D_1} E(\hat{x}), \nabla_{D_2} E(\hat{x}),  \nabla_{D_3} E(\hat{x}),  \nabla_{D_4} E(\hat{x})\}. \\
=\left\{\sum_{i=1}^4\lambda_i \nabla_{D_i} E(\hat{x}), \sum_{i=1}^4 \lambda_i=1 \text { and } \lambda_i \geq 0\right\}
\end{array}
\end{equation}
The generalized directional derivative $E^o(x, h(\hat{x}))$ evaluated in $\hat{x}$ where $E$ is not differentiable is defined as 
\begin{equation}
\begin{array}{r}
E^o(\hat{x}, h(\hat{x}))=\max \{\langle\xi, h(\hat{x})\rangle, \quad \xi \in \partial E(\hat{x})\}. \\
= \max\left\{\langle\sum_{i=1}^4\lambda_i \nabla_{D_i} E(\hat{x}), h(\hat{x})\rangle,\ \sum_{i=1}^4 \lambda_i=1, \ \lambda_i \geq 0\right\} \leq 0. \\
= \max\{\langle \nabla_{D_i} E(\hat{x}), h(\hat{x})\rangle,\ i=1, 2, 3, 4\}
\end{array}
\label{eq:generalized_lie_derivative}
\end{equation}
Therefore, $E^o(x, h(x))\leq 0$ for all $x$ in the state space and we can conclude that the energy function $E^o(x, h(x))$ is non-increasing along the forward trajectories of the system in  \eqref{eq:autonomous_limit}.
\paragraph{Lasalle's Analysis }
According to Theorem \ref{thm:lasalle_nonsmooth} all trajectories converge to the largest invaraint set in $\mathcal{S}=\left\{x \in \mathcal{B}: E^o(x, h(x))=0\right\}$. In the following we show that this set is the set of equilibria. The set $\mathcal{S}$ is the union of three different components:
\begin{itemize}
\item $ \mathcal{S}_{\text{eq}} = \{x:\ h(x)=0\}$, the set of equilibrium points;

\item $	\mathcal{S}_{\text{sat}} = \overline{\{x\in \mathcal{S}: \frac{\partial}{\partial x_1}g_1(x_1)= 0 \land \frac{\partial}{\partial x_2}g_2(x_2)=0 \}}$\footnote{\label{note1} We consider the closure of the set, including boundary points where $g_i$ are not differentiable, but the corresponding generalized derivative remains zero.},  the set of points where both activation functions are constant;

\item  $\mathcal{S}_{\text{mix}} = \overline{\{x\in \mathcal{S}: \frac{\partial}{\partial x_1}g_1(x_1) \frac{\partial}{\partial x_2}g_2(x_2)=0,\  \frac{\partial}{\partial x_1}g_1(x_1) \neq\frac{\partial}{\partial x_2}g_2(x_2) \}}$, the set of points where only one of the activation functions is constant.
\end{itemize}
A simplified, intuitive visualization of the sets $\mathcal{S}{\text{eq}}, \mathcal{S}{\text{sat}}, \mathcal{S}_{\text{mix}}$ can be seen in Figure \ref{fig:domain_example}. $\mathcal{S}_{\text{eq}} \subset \mathcal{M}$ as equilibria are clearly invariant. We proceed to demonstrate that in both $\mathcal{S}_{\text{sat}}$ and $\mathcal{S}_{\text{mix}}$, the only invariant sets are the equilibria. The proof for $\mathcal{S}_{\text{sat}}$ is presented here, as the proof for $\mathcal{S}_{\text{mix}}$ follows a similar logic.

The set $\mathcal{S}_{\text{sat}}$ can be obtained as the disjoint union of sets of the form $[a_i^1, b_i^1] \times [a_i^2, b_i^2]$ where $a_i^1 \leq b_i^1$ and $a_i^2 \leq b_i^2$. 
\begin{equation}
\mathcal{S}_{\text{sat}} = \bigcup\limits_{i}\ [a_i^1, b_i^1] \times [a_i^2, b_i^2]
\end{equation}
The dynamics, restricted to each of these sets $\ [a_i^1, b_i^1] \times [a_i^2, b_i^2]$ has the form
\begin{equation}
\begin{aligned}
\dot{x}_1 = -\gamma_{1} x_1 +c_1 \\
\dot{x}_2 = -\gamma_{2}x_2 +c_2 
\end{aligned}.
\label{eq:pwa_restriced_sat}
\end{equation}
Assume $x^* = [x^*_1, x^*_2]\in [a_i^1, b_i^1] \times [a_i^2, b_i^2]$ is not an equilibrium, then there exists $\tilde{t} \in$ $(-\infty,+\infty)$ such that \textcolor{black}{$\phi\left(\tilde{t}, x^*\right) \notin [a_i^1, b_i^1] \times [a_i^2, b_i^2]$} and $\phi\left(\tilde{t}, x^*\right) \notin \mathcal{S}_{\text{sat}}$ as the only invariant set under the dynamics in \eqref{eq:pwa_restriced_sat} in $[a_i^1, b_i^1] \times [a_i^2, b_i^2]$ is the set of equilibria.




\begin{figure}
\centering
\includegraphics[width=0.95\linewidth]{domain_representation}
\caption{Graphical visualization of the sets $\mathcal{S}_{\text{eq}}, \mathcal{S}_{\text{sat}}, \mathcal{S}_{\text{mix}}$ for a bistable system like \eqref{eq:autonomous_limit} where both $g_1$ and $g_2$ are piecewise affine functions.}
\label{fig:domain_example}
\end{figure}




%\begin{equation}
%	\mathcal{S}_{p\text{eq}} = \{x\in \mathcal{S}: h_1(x)\neq 0 \lor  h_2(x)\neq 0 \}
%\end{equation}
%	, i.e. the set of non equilibrium points where the generalized directional dertivative of the energy function $E^o(x, h(x))$ along the vector field $h(x)$ is zero. 


\iffalse
$$
\mathcal{S}=\left(\cup_{\alpha \in \Lambda_e} \Omega_\alpha\right) \cup\left(\cup_{\alpha \in \Lambda^m} I_\alpha\right) \cup \mathcal{E}_0
$$
where:
\begin{itemize}
\item $\cup_{\alpha \in \Lambda_c} \Omega_\alpha$ is the union of all saturated regions. Indeed, for all $x \in \cup_{\alpha \in \Lambda_e} \Omega_\alpha$, no species $x_{i, j}$ is in the linear region, therefore according to (24) $E^o(x, F(x))=$ $0, \forall x \in \cup_{\alpha \in \Lambda_e} \Omega_\alpha$.
\item $\cup_{\alpha \in \Lambda_m} I_\alpha$ is the union (by definition), over all the mixed regions, of the subsets $I_\alpha$ where the components of the vector field corresponding to the species in the linear region vanish. Therefore the sum in (24) has all terms equal to zero.
\item $\mathcal{E}_0$ is the set of equilibria in the linear region. Indeed, the only points in the interior domain such that $E^o(x ; F(x))=0$ are the equilibria (the square of all the entries of the vector field $F(x)$ has to be zero).
\end{itemize}

\fi
We proved that all trajectories of the limiting autonomous vector field \eqref{eq:autonomous_limit} converge to one equilibrium, and that the equilibria are isolated. Furthermore, no equilibria are 

we can conclude that for all forward trajectories that synchronize, every compartment converges to the same equilibrium point $P$. Notably, this point $P$ is also an equilibrium of the isolated compartment (Corollary \ref{corollary_main_equilibria}, Appendix C).
\end{proof}


